AI for Open Science: A Multi-Agent Perspective for Ethically Translating Data to Knowledge

AI for Science (AI4Science), particularly in the form of self-driving labs, has the potential to sideline human involvement and hinder scientific discovery within the broader community. While prior research has focused on ensuring the responsible deployment of AI applications, enhancing security, and ensuring interpretability, we also propose that promoting openness in AI4Science discoveries should be carefully considered. In this paper, we introduce the concept of AI for Open Science (AI4OS) as a multi-agent extension of AI4Science with the core principle of maximizing open knowledge translation throughout the scientific enterprise rather than a single organizational unit. We use the established principles of Knowledge Discovery and Data Mining (KDD) to formalize a language around AI4OS. We then discuss three principle stages of knowledge translation embedded in AI4Science systems and detail specific points where openness can be applied to yield an AI4OS alternative. Lastly, we formulate a theoretical metric to assess AI4OS with a supporting ethical argument highlighting its importance. Our goal is that by drawing attention to AI4OS we can ensure the natural consequence of AI4Science (e.g., self-driving labs) is a benefit not only for its developers but for society as a whole.

==> Sections/discovery_support.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=.9\textwidth]{Figures/agent_knowledge_flow.png}
    \caption{A knowledge flow diagram between three critical teams in the knowledge translation process. Each variable $k$ represents a knowledge base of each respective team in the process such that $\overline{k_i}$ denotes all the knowledge of the experimenting team responsible for collecting a dataset, $\underline{k_j}$ denotes the knowledge of the data mining team responsible for KDD steps 1-7, and $\widecheck{k}_l$ represents the knowledge of the labeling team. $k_{ijl}$ is the new knowledge that is labeled by the labeling team and numbers 1-4 label the four potential communication flows that can occur between the agents, not including potential loops.}
    \label{fig:knowledge_flow}
\end{figure*}

\section{Enhancing Discovery Support with Data and Information Provenance}

We define a Discovery Support System (DiSS) as:
\begin{quote}
    An AI system that supports the generation of useful hypotheses that aid in labeling new knowledge in-line with the set of true knowledge $K$.
\end{quote}

In science, the knowledge translation process is inherently disjointed, involving multiple agent collaborators and knowledge sharing. This is because the same agent will likely not perform, or even be included, in all steps of the knowledge translation process, i.e., the process by which raw data is collected via experimentation, mined for patterns to create information, which is then interpreted knowledge through appropriate labeling. For instance, you may have a biomedical research team that decides to collect genomics data on breast cancer patients. This team designs the experiments, selects the population, and performs data aggregation. As is now common in the biomedical and machine learning community, this research team then makes this dataset open to others. Then, a separate data mining team then consumes this open data and extracts potential patterns to form a set of information. From this point a separate labeling team, such as a team of oncologists, are presented with this mined information and asked to assign labels to any potential new knowledge derivable from that information. As such, it can be helpful to consider a DiSS system as a collaborative team effort where each team (composed of humans, machines or a mix) has a duty to "aid in the labeling of new knowledge" by transferring their prior knowledge, used in their contribution to the knowledge translation process, to downstream teams. Moreover, while we argue that it is ethically imperative for teams to transfer their prior knowledge to downstream teams, we also recognize a duty for teams to ingest prior knowledge from their peers and ensure it is, "in-line with the set of true knowledge $K$", or more likely, their approximation of $K$. We draw from this intuition when deriving our objective function for DiSS in Section 4.

Unlike the days of Swanson \cite{swanson_fish_1986}, high degrees of domain specialization exacerbates the need for diverse teams. Each team has different domain knowledge related to their disciplines, world knowledge based on their lived experiences, as well as knowledge of assumptions regarding potential biases introduced into their particular step of the knowledge translation process. For instance, the experimenting team may have selected patients with a demographic bias based on the team's geographical location. The data mining team may have selected a novel normalization step based on their mining experience of similar datasets skewing the information obtained. Further still, the knowledge labeling team may have a particular self-affirming bias toward research and findings they hope to see or deduce from the mined information. 

In any case, it is clear knowledge sharing between these teams is essential for appropriate knowledge labeling. Figure \ref{fig:knowledge_flow} depicts the primary channels of knowledge flow between these various teams. Channel 1 represents the communication between the experimenting team and data mining team regarding the data collection and experimental design assumptions present in a dataset. Naturally, the more knowledge the data mining team has in regards to $\overline{k_i}$, the more contextualized the mined information will become. Channel 2 corresponds to the knowledge flow of algorithmic bias, model selection, etc., including domain and world knowledge of the data mining team to the knowledge labeling team. This allows the labeling team to review potential bias avoiding knowledge labeling mishaps. Similarly, channel 3 fosters the communication of knowledge from the experimenting team to the labeling team, allowing the labeling team to account for any biases that yield the mined information. Lastly, channel 4 (a culmination of channels 1-3) depicts the ideal knowledge flow such that the labeling team has access to the knowledge bases of both the experimenting team and the data mining team and the data mining team has access to the knowledge base of the experimenting team. Naturally, it is also possible for teams to develop simultaneous nested knowledge translation processes such that their individual knowledge bases are also increasing over time. In other words, this knowledge flow need not be static and may contain loops such that agents can update and refine their own knowledge bases at will.

These four channels illustrate the need for data and information provenance, i.e., origination knowledge, that allows each team to make the best decisions at each point in the process. In the next section, we will take these general intuitions and form a concrete framework for knowledge translation based on team communication throughout the knowledge process. This will culminate in a clear argument validating these ideas in terms of the amount of new knowledge generation and yield technical and societal solutions recommendations for implementing these communication channels ethically and robustly.

==> Sections/future_work.tex <==
\section{Implementation Recommendations for Future Work}
Our KTF is meant to serve as a foundational approach that depicts the collaborative and interoperable translation processes of data to information to knowledge. While the KDD process has been considered from a multi-agent perspective \cite{pop_multi-agent_2006,kadar_automated_2017}, to the best of our knowledge this framework is the first to formalize knowledge discovery from both a multi-agent perspective as well as accounting for prior knowledge propagation along each step of agent role hierarchy. While this framework is designed to be generalizable, there are still gaps we wish to address. In short, these are as follows:

\begin{enumerate}
    \item Provide technical solutions to the knowledge transfer problem among the collaborative teams of the knowledge translation processes,
    \item Relax the assumed rectified team knowledge priors and formalize the process of how their knowledge is rectified (or not) for a team,
    \item Formalize qualitative success for the knowledge translation process.
\end{enumerate}

Our first point stems from the issue of knowledge transfer between the \textit{experimenting, data mining} and \textit{labeling teams}. We showed that these prior knowledge sets form monotonic relationships over resulting information, ultimately leading to the objective of DiSS in Equation \ref{eq:diss_goal}. We discussed societal implications of the knowledge transfer problem (equitable access to DiSS systems and siloing knowledge within organizations) and even further societal solutions to the knowledge transfer problem (legislation in support of Open Science principles, provenance chains maintained by researchers and educating researchers to rigorously test new knowledge). However, the question remains, to what extent can knowledge transfer be automated. We discussed before ``datasheets for datasets" \cite{gebru_datasheets_2021} as a way to have authors produce questionnaires related to intent, composition, collection, use, distribution and maintenance. What would it look like for a system to automate this processes and require subsequent teams to respond to these questionnaires before accessing data. We provide no technical solutions to this problem, allowing this to be extended in the future.

Our second point stems from our assumption of rectified knowledge. While it is ideal for teams to agree on all prior knowledge on experimenting, mining, and labeling, it is likely in practice that among teams there will be conflict whether or not they are aware of it. Further, not every agent is guaranteed to influence each aspect of experimenting, mining or labeling. One agent might employ knowledge from $K^c$ on some aspect of the experimenting processes, while another would have employed knowledge from $K$, but because their jobs were partitioned, no rectification would have occurred. For this reason it is relevant to consider instances where teams may or may not be able to rectify knowledge. We think that framing this under the perspective of measuring interference (positive or negative) \cite{hoc_towards_2001} would be readily digestible into the DiSS framework.

Our final point stems from the need to access a DiSS qualitatively. For example, Cooke et al. \cite{cooke_measuring_2003} measures team knowledge after applying a knowledge transfer process called cross-training (hands-on practice of tasks from other team members) and conceptual cross-training (sharing of mental models from the perspective of team-member roles). However, there is a need for automated frameworks to accomplish such evaluations of a DiSS. Further, these assessment strategies should capture some sense of Value-Sensitive Design so that DiSS aligns with appropriate ethical considerations. In other words, the quality of a DiSS should measure whether or not human values are either supported or diminished by a particular
design \cite{cummings_integrating_2006}. This suggests the need for evaluating over benchmark datasets that span ethical considerations like labeling of hate speech \cite{elsherief_latent_2021} or concepts such as justice, well-being, duties, virtues, and commonsense morality \cite{hendrycks_aligning_2020}.
